Motion-Based Generator Model: Unsupervised Disentanglement of Appearance, Trackable and Intrackable Motions in Dynamic Patterns

Dynamic patterns are characterized by complex spatial and motion patterns. Understanding dynamic patterns requires a disentangled representational model that separates the factorial components. A commonly used model for dynamic patterns is the state space model, where the state evolves over time according to a transition model and the state generates the observed image frames according to an emission model. To model the motions explicitly, it is natural for the model to be based on the motions or the displacement fields of the pixels. Thus in the emission model, we let the hidden state generate the displacement field, which warps the trackable component in the previous image frame to generate the next frame while adding a simultaneously emitted residual image to account for the change that cannot be explained by the deformation. The warping of the previous image is about the trackable part of the change of image frame, while the residual image is about the intrackable part of the image. We use a maximum likelihood algorithm to learn the model that iterates between inferring latent noise vectors that drive the transition model and updating the parameters given the inferred latent vectors. Meanwhile we adopt a regularization term to penalize the norms of the residual images to encourage the model to explain the change of image frames by trackable motion. Unlike existing methods on dynamic patterns, we learn our model in unsupervised setting without ground truth displacement fields. In addition, our model defines a notion of intrackability by the separation of warped component and residual component in each image frame. We show that our method can synthesize realistic dynamic pattern, and disentangling appearance, trackable and intrackable motions. The learned models are useful for motion transfer, and it is natural to adopt it to define and measure intrackability of a dynamic pattern.

==> sections/theory.tex <==
\section*{Appendix: Theoretical understanding}

\subsection*{Kullback-Leibler divergence} 

The Kullback-Leibler divergence between two distributions $p(x)$ and $q(x)$ is defined as ${\rm KL}(p\|q) = \E_{p}[\log (p(X)/q(X))]$. 

The Kullback-Leibler divergence between two conditional distributions $p(y|x)$ and $q(y|x)$ is defined as 
\begin{eqnarray}
    {\rm KL}(p\|q) &=& \E_p\left[\log \frac{p(Y|X)}{q(Y|X)}\right] \\
    &=& \int \log \frac{p(y|x)}{q(y|x)} p(x, y) dxdy, 
 \end{eqnarray}
 where the expectation is over the joint distribution $p(x, y) = p(x) p(y|x)$. 

\subsection*{Slow thinking planner-like model} 

The slow thinking planner-like model is
\begin{eqnarray} 
   p(Y|C; \theta) = \frac{p(Y,C;\theta)}{p(C;\theta)}
   =\frac{p(Y,C;\theta)} {\int p(Y,C; \theta) dY} \nonumber\\ 
   =\frac{1}{Z(C; \theta)} \exp \left[ f(Y,C; \theta)\right], \label{eq:D1}
\end{eqnarray}  
where 
\begin{eqnarray} 
    Z(C; \theta) = \int \exp \left[ f(Y,C; \theta)\right] dY
\end{eqnarray}
is the normalizing constant and is analytically intractable. 

Suppose the training examples $\{(Y_i, C_i), i = 1, ..., n\}$ are generated by the true joint distribution $f(Y, C)$, whose conditional distribution is $f(Y|C)$. 

For large sample $n \rightarrow \infty$, the maximum likelihood estimation of $\theta$ is to minimize the Kullback-Leibler divergence 
\begin{eqnarray}
\min_\theta  {\rm KL}(f(Y|C)\| p(Y|C; \theta)). 
\end{eqnarray} 
In practice, the expectation with respect to $f(Y, C)$ is approximated by the sample average. The difficulty with $ {\rm KL}(f(Y|C)\| p(Y|C; \theta))$ is that the $\log Z(C; \theta)$ term is analytically intractable, and its derivative has to be approximated by MCMC sampling from the model $p(Y|C; \theta)$. 

\subsection*{Fast thinking policy-like model} 

The fast thinking policy-like model is 
\begin{eqnarray} 
  X \sim \N(0, I_d),  \;  Y = g(X, C; \alpha) + \epsilon,  \; \epsilon \sim \N(0, \sigma^2  I_D).   \label{eq:G1}
 \end{eqnarray}
 We use the notation $q(Y|C; \alpha)$ to denote the resulting conditional distribution. It is obtained by 
\begin{eqnarray} 
    q(Y|C; \alpha) = \int q(X) q(Y|X, C; \alpha) dX, 
 \end{eqnarray} 
 which is analytically intractable. 
 
 For large sample, the maximum likelihood estimation of $\alpha$ is to minimize the Kullback-Leibler divergence 
\begin{eqnarray}
\min_\alpha  {\rm KL}(f(Y|C)\| q(Y|C; \alpha)). 
\end{eqnarray} 
Again, the expectation with respect to $f(Y, C)$ is approximated by the sample average. The difficulty with ${\rm KL}(f(Y|C)\| q(Y|C; \alpha))$ is that $\log q(Y|C; \alpha)$ is analytically intractable, and its derivative has to be approximated by MCMC sampling of the posterior $q(X|Y, C; \alpha)$. 

\subsection*{Value shift: modified contrastive divergence} 

 Let $M(Y_1|Y_0, C; \theta)$ be the transition kernel of the finite-step MCMC that refines the initial solution $Y_0$ to the refined solution $Y_1$. Let $(M_\theta q)(Y_1|C; \alpha) = \int M(Y_1|Y_0, C; \theta)  q(Y_0|C; \alpha) dY_0$ be the distribution obtained by running the finite-step MCMC from $q(Y_0|C; \alpha)$. 
 
 Given the current policy-like model $q(Y|C; \alpha)$, the value shift updates $\theta_t$ to $\theta_{t+1}$, and the update approximately follows the gradient of the following modified contrastive divergence \cite{Hinton2002a, xie2016cooperative}
 \begin{align}
 &{\rm KL}(f(Y|C)\| p(Y|C; \theta)) \nonumber \\- &{\rm KL}((M_{\theta_t} q)(Y|C; \alpha)\| p(Y|C; \theta)). \label{eq:MCD}
\end{align} 
Compare (\ref{eq:MCD}) with the MLE (\ref{eq:D1}),  (\ref{eq:MCD}) has the second divergence term $ {\rm KL}((M_{\theta_t} q)(Y|C; \alpha)\| p(Y|C; \theta))$ to cancel the $\log Z(C; \theta)$ term, so that its derivative is analytically tractable. The learning is to shift $p(Y|C; \theta)$ or its high value region around the mode from the refined solution provided by $(M_{\theta_t} q)(Y|C; \alpha)$ toward the observed solution given by $f(Y|C)$. If $(M_{\theta_t} q)(Y|C; \alpha)$ is close to $p(Y|C; \theta)$, then the second divergence is close to zero, and the learning is close to MLE update. 

\subsection*{Mapping shift: distilling MCMC} 

Given the current planner-like model $p(Y|C; \theta)$, the mapping shift updates $\alpha_t$ to $\alpha_{t+1}$, and the update approximately follows the gradient of 
 \begin{eqnarray}
 {\rm KL}((M_\theta q)(Y|C; \alpha_{t})\| q(Y|C; \alpha)). \label{eq:DM}
\end{eqnarray} 
This update distills the MCMC transition $M_\theta$ into the model $q(Y|C; \alpha)$.  In the idealized case where the above divergence can be minimized to zero, then $q(Y|C; \alpha_{t+1}) = (M_\theta q)(Y|C; \alpha_{t})$. The limiting distribution of the MCMC transition $M_\theta$ is $p(Y|C; \theta)$,  thus the cumulative effect of the above update is to lead $q(Y|C; \alpha)$ close to $p(Y|C; \theta)$. 

Compare (\ref{eq:DM}) to the MLE (\ref{eq:G1}), the training data distribution becomes $(M_\theta q)(Y|C; \alpha_{t})$ instead of $f(Y|C)$. That is, $q(Y|C; \alpha)$ learns from how $M_\theta$ refines it. The learning is accomplished by mapping shift where the generated latent vector $X$ is known, thus does not need to be inferred (or the Langevin inference algorithm can initialize from the generated $X$). In contrast, if we are to learn from $f(Y|C)$, we need to infer the unknown $X$ by sampling from the posterior distribution. 

In the limit, if the algorithm converges to a fixed point, then the resulting $q(Y|C; \alpha)$ minimizes  ${\rm KL}((M_\theta q)(Y|C; \alpha)\| q(Y|C; \alpha))$, that is, $q(Y|C; \alpha)$ seeks to be the stationary distribution of the MCMC transition $M_\theta$, which is $p(Y|C; \theta)$. 

If the learned $q(Y|C; \alpha)$ is close to $p(Y|C; \theta)$, then $(M_{\theta_t} q)(Y|C; \alpha)$ is even closer to $p(Y|C; \theta)$. Then the learned $p(Y|C; \theta)$ is close to MLE because the second divergence term in (\ref{eq:MCD}) is close to zero. 



